Analyzing Flowgraphs with ATL

This paper presents a solution to the Flowgraphs case study for the Transformation Tool Contest 2013 (TTC 2013). Starting from Java source code, we execute a chain of model transformations to derive a simplified model of the program, its control flow graph and its data flow graph. Finally we develop a model transformation that validates the program flow by comparing it with a set of flow specifications written in a domain specific language. The proposed solution has been implemented using ATL.

==> eptcsdata.tex <==
\providecommand{\firstpage}{32}
\providecommand{\publicationstatus}{Pieter Van Gorp, Louis M. Rose, Christian Krause (Eds.):\\
Sixth Transformation Tool Contest (TTC 2013)\\
EPTCS 135, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.135.4}{10.4204/EPTCS.135.4}}
\pdfoutput=1

